Towards a Performance Model for Byzantine Fault Tolerant (Storage) Services

Byzantine fault-tolerant systems have been researched for more than four decades, and although shown possible early, the solutions were impractical for a long time. With PBFT the first practical solution was proposed in 1999 and spawned new research which culminated in novel applications using it today. Although the safety and liveness properties of PBFT-type protocols have been rigorously analyzed, when it comes to practical performance only empirical results - often in artificial settings - are known and imperfections on the communication channels are not specifically considered. In this work we present the first performance model for PBFT specifically considering the impact of unreliable channels and the use of different transport protocols over them. We also did extensive simulations to verify the model and to gain more insight on the impact of deployment parameters on the overall transaction time. We show that the usage of UDP can lead to significant speedup for PBFT protocols compared to TCP when tuned accordingly even over lossy channels. Finally, we compared the simulation to a real implementation and measure the benefits of a developed improvement directly. We found that the impact on the design of the network layer has been overlooked in the past but offers some additional room for improvement when it comes to practical performance. In this work we are focusing on the optimistic case with no node failures, as this is hopefully the most relevant situation.

==> conference/sections/service.tex <==
\section{Robust Multi-Cloud Storage (with Security)}
\label{sec:service_implementation}

SERDS functionality is split up into client-side and server-side logic as despicted in Figure~\ref{fig:overview_service}. The client-side module provides privacy and security by generating secret shares which are distributed among the selected cloud providers (constituting the depicted privacy layer). In addition, we provide a module for cloud providers which provides protocols for guaranteeing robustness, availability and consistency among the employed cloud providers (constituting the depicted consistency layer).

Both modules are loosely coupled such that each of them can be independently used by third party software. Allowing third parties to provide their own solution for maintaining high availability or confidentiality. 
To achieve this, both modules provide a RESTful API and are implemented in JavaScript where, stand-alone parts use node.js~\cite{url:NODEJS}.

%%
%\begin{figure}
%\includegraphics[scale=0.6]{figures/service_overview.pdf}
%\caption{SERDS with its layers and the cloud-of-clouds.}
%\label{fig:overview_service}
%\end{figure}
%%

\todo[inline]{Introduce architecture with consistency layer, and privacy layer}

%\subsection{Consistency Layer}
%\label{sec:bft-node}

As a basis for our \textit{consistency layer} we use a modified version of the PBFT protocol introduced by~\cite{Castro:1999:PBF}. PBFT is based on a network model with only weak synchrony and has only three phases of overhead.
It is the best suited solution for our relatively static scenario with a rather manageable amount of network nodes and good connectivity between them. However, the protocol foresees that each replica holds the identical data, which may not be the case depending on the algorithms/protocols used in the privacy layer.
The problems that arise when using PBFT and secret sharing have already been briefly discussed in~\cite{Happe:2017:malicious} which also provides an initial solution. In the following we provide improved solutions for the following identified issues in~\cite{Happe:2017:malicious}.

In case of secret sharing each replica may hold a different share, thus invalidating the aforementioned assumption of PBFT. 
So, replicas cannot generate a hash using the provided data for the PBFT protocol. 
In order to cope with this limitation we introduce meta-data which sole purpose is to have some static data among the generated shares. 
This meta-data could be purely random. This solves three issues mentioned in~\cite{Happe:2017:malicious}, namely~\textbf{Matching Client-Requests},~\textbf{Verifying operation results} and~\textbf{Checkpointing protocol}. 
%
\begin{figure}[tbh!]
\centering
\includegraphics[width=0.4\textwidth]{figures/pbft}
\caption{Message flow diagram of PBFT with the extended first phase. Altered phases and communications are highlighted by red.}
\label{fig:msg-flow}
\end{figure}

\textbf{Matching Client-Requests.} Figure~\ref{fig:msg-flow} depicts the extended PBFT as proposed in~\cite{Happe:2017:malicious}. 
In contrast to the original PBFT algorithm, each replica temporary stores the received request but as specified only the primary broadcasts the pre-prepare messages accompanied with the hash of the received meta-data. 
In addition to the conditions that must hold for PBFT (received messages must be authentic, digests must match among at least $2f + 1$ received messages) that a replica only enters the prepare phase if it has received a corresponding request. 
On successful commit, each replica stores the initially received meta-data and secret share in its content store.

\textbf{Verifying operation results.} Having the same meta-data stored by each replica, clients are able to judge whether a request has been successfully executed (esp. in the case of a read request). 
Each replica sends upon a successful commit its secret share and meta-data to the requesting client. The client can then verify the result given the meta-data without reconstructing the secret. 
Therefore, we modify the last phase of the PBFT protocol depicted in Figure~\ref{fig:msg-flow} by red arrows.

\textbf{Checkpointing protocol}. Since secret shares are usually of identical length one may employ a weighted checksum, checking whether all replicas are holding the same data. 
Otherwise, the meta-data could be used to apply a weighted checksum approach.


Our approach also incorporates a \textit{privacy layer} and uses secure data fragmentation based on secret sharing to build secure multi-cloud storage systems on top of single cloud storage offerings.
Using secret sharing instead of other techniques like replication or erasure coding provides additional confidentiality for stored data without the use of additional encryption.
SERDS support three types of encoding, i.e., perfectly secure secret sharing~\cite{shamir79} and computational secure secret sharing~\cite{krawcz93}, as well as information dispersal.
We focus on secret sharing schemes with threshold access structures, because they are the most efficient and practical solutions for storage systems and provide the $k$-out-of-$n$ behavior known from erasure coding and lead to very efficient storage systems when the computational secure version is used.

%\textit{Perfectly secure secret sharing (PSS)} is instantiated by Shamir secret sharing~\cite{shamir79}.
%This version has many desirable properties and is well suited for both, software and hardware implementation, especially if small message spaces can be used.
%It is perfectly secure, because it gives information theoretical guarantees, i.e., when the receiver has less than $k$ shares available even unbounded adversaries are not able to recover the plaintext.
%Additionally, secret sharing schemes can assure integrity of stored data if more than $k$ shares are available for reconstruction through their inherent redundancy.
%However, their drawback is the achievable information rate.
%For perfect security each share needs to be as long as the original file which makes the scheme very inefficient for storage applications. In fact, the scheme is even less storage efficient than pure replication.
%
%To enable more efficient storage solutions SERDS also supports~\textit{Information Dispersal (IDS)}. IDS is using non-systematic erasure coding to generate data fragments for distribution.
%It does not give any security guarantees, but produces the shortest possible fragments together with a $k$-out-of-$n$ access structure to increase availability of data.
%The integrity properties are identical to the PSS scheme.
%
%However, if both schemes ---PSS and IDS--- are combined \textit{Computational Secret Sharing (CSS)} can be build. The combination was first proposed by Krawczyk~\cite{krawcz93} and enables efficient and secure storage of data. On a high level, the plaintext data is encrypted using a symmetric encryption scheme, and then the secret sharing scheme is applied the used key and the information dispersal scheme to the resulting ciphertext. 
%
%In general, no matter if secret sharing or erasure coding is used, both modes introduce similar challenges for BFT systems because they do not replicate data but encoded fragments which are different on each storage node.
%However, in the case of secret sharing the security has to be always considered in the protocol design, and fragments of data objects must not be exchanged between servers, which makes the protocol integration even harder.
%SERDS tries to keep the dependencies between the privacy and the consistency layer as small as possible to also enable independent use.
%However, due to some peculiarities this can only be done to a certain extend. 
%Furthermore, for optimal protocol performance the following considerations have to be addressed in the full system.

\begin{table}[tbh!]
\centering
\begin{tabular}{c|c|c|c|c|c|c|}
  \cline{2-7}
  & \multicolumn{2}{c|}{PSS} & \multicolumn{2}{c|}{IDS} & \multicolumn{2}{c|}{CSS} \\ \cline{2-7}
  &  Enc & Dec & Enc & Dec & Enc & Dec \\ \cline{1-7}
  \multicolumn{1}{|c|}{Java~\cite{Loruenser:2015:ARCHISTAR}} & 22.2 & 21.9 & 169.2  & 58.2 & 67.1 & 38.9 \\ \cline{1-7}
  \multicolumn{1}{|c|}{JS naive} & 0.1 & 2.3 & 5.5 & 5.3 & 2.8 & 2.6 \\ \cline{1-7}
  \multicolumn{1}{|c|}{JS~[This work]} & 6.5 & 28.1 & 67.1  & 61.0 & 38.9 & 36.9 \\ \cline{1-7}
\end{tabular}
\caption{Performance comparison of SERDS privacy layer in JavaScript (JS) with Archistar-Smc Java implementation taken on a Core2 Duo E8400 @ 3.00GHz running Ubuntu16.4, Java8 and Node.js 4.2.6. All values in MB/s.}
\label{tab:secret_sharing}
\end{table}

%The idea of SERDS is to shift the fragmentation of data to the client.
%This has a positive impact on the security and solves the issue of having a single point of trust from the system.
%In order to support this idea and allow for the broadest proliferation of the technology JavaScript was selected for implementation, thus enabling web based clients.
%Performance of JavaScript is often a problem for cryptographic algorithms~\cite{Stark2009} and initially prevented us from its use for storage applications.
%However, there are ways to achieve competitive performance on JavaScript platforms by, i.e., the use of~\textit{asm.js}\footnote{http://asm.js, accessed 19.6.2018.}.
%By using~\textit{emscripten}\footnote{http://emscripten.org, accessed 19.6.2018.} C/C++ code can be compiled down to a very restricted subset of JavaScript to be executed very efficiently by modern JavaScript VMs. 
%Following this approach and after additional handwritten JavaScript optimizations the solutions are now an order of magnitude faster than the naive implementations and in the range of optimized Java implementations.
%%, with the exception of CSS, which is slower due to the use of a slow underlying cipher used for encryption.
%Furthermore, PSS was not implemented in asm.js.
%It is only used for sharing the keys in CSS method, which are small compared to the payload data in the protocol.

The use of a privacy layer comes almost for free in terms of storage overhead and introduces only limited 
We measured the performance achieved for 
The resulting performance is shown in Table~\ref{tab:secret_sharing} and compared to a naive implementation as well as comparable Java solution.
The throughput for secure encoding type CSS in Javascript is about 60\% of the speed of erasure coding wiht IDS and roughly the same compared to optimized Java implementations, i.e., it does not limit the overall performance especially as this can easily be parallelzied on a transaction level.


%However, to relax the trust assumptions about clients it must be assured that the data stored in the system is consistent. For the storage application, this means that the system has to guarantee that not only the meta-data but also the shares are consistent. To achieve this we integrated the idea of fingerprinting for CSS~\cite{krawcz93} into our system. For CSS-encoded data the digest values of all shares are added to the meta-data. Therefore, the BFT nodes can check if their shares are consistent with the digest of the transaction data and stop if they detect any inconsistency. The same method works for erasure coded data. For PSS we propose the adaption of an auditing protocol presented in~\cite{todo} which is integrated into the BFT phases. The method based on fingerprinting must not be used because the digest leaks information about the shares which is not allowed for perfect security. In addition to the digest about the meta-data a weighted sum over the shares is also included. For efficiency reasons, we only recommend the use of the PSS algorithm for very sensitive data with highest confidentiality requirements and suggest to use CSS for bulk data.

%The read operations have to be modified for usage by the privacy layer. For CSS data the meta-data have to be reconstructed by a majority decoding of ``2f+1'' answers. Afterwards, the received shares are validated against the digest included in the meta-data. If they are valid, they are included in the reconstruction algorithm. From the guarantees given by the consistency layer it is easy to see the composed system fulfills all criteria of the consistency layer and constitutes therefore an optimal integration. In the case of PSS data the situation is different. Given the fact, that PSS is only $3f+1$ robust, the reconstruction must involve at least $f$ answers more compared to majority voting. Although $2f+1$-robust schemes exist, but they cannot be integrated with BFT as CSS presented above. Therefore, if pure PSS must be supported by the system $4f+1$ nodes must be available for operation.

%In summary, most of the functionality can be implemented on the privacy layer, but still the consistency layer has to be aware of the encoding types of data and treat them differently, i.e., they can not be abstracted away.
%Additionally, the type of data has also an influence on the robustness guarantees.


